How to Safely Use Extensionality in Liquid Haskell

Refinement type checkers are a powerful way to reason about functional programs. For example, one can prove properties of a slow, specification implementation, porting the proofs to an optimized implementation that behaves the same. Without functional extensionality, proofs must relate functions that are fully applied. When data itself has a higher-order representation, fully applied proofs face serious impediments! When working with first-order data, fully applied proofs lead to noisome duplication when using higher-order functions. While dependent type theories are typically consistent with functional extensionality axioms, refinement type systems with semantic subtyping treat naive phrasings of functional extensionality inconsistently, leading to unsoundness. We demonstrate this unsoundness and develop a new approach to equality in Liquid Haskell: we define a propositional equality in a library we call PEq. Using PEq avoids the unsoundness while still proving useful equalities at higher types; we demonstrate its use in several case studies. We validate PEq by building a small model and developing its metatheory. Additionally, we prove metaproperties of PEq inside Liquid Haskell itself using an unnamed folklore technique, which we dub `classy induction'.

==> ext-typing.tex <==
%auto-ignore
\begin{figure}
\small
\noindent \textit{Sybtyping Rules}\hfill
\vspace*{0.1em}
$$
\inference{    
    \text{``top-level-refinements of }\env\text{''} \land r_1 \Rightarrow r_2
}{
    \issubtype{\env}{\{v:\alpha \mid r_1\}}{\{v:\alpha \mid r_2\}}
}[\subgbase]
\quad
\inference{    
    \issubtype{\env}{\typ'_x}{\typ_x} && 
    \issubtype{\env, \envBind{x}{\typ'_x}}{\typ}{\typ'}
}{
    \issubtype{\env}{\tfun{x}{\typ_x}{\typ}}{\tfun{x}{\typ'_x}{\typ'}}
}[\subgfun]
$$

\vspace*{0.5em}
\noindent \textit{Subtyping Derivation Leaves}\hfill
\vspace*{0.1em}
\begin{adjustbox}{max size={\textwidth}{\textheight}}
$$
\inference{
    \inference{
        \apred \Rightarrow \hdom
    }{
    \issubtype{\env}{\tya}{\{v:\alpha \mid \hdom\}}
     } && 
     \inference{
        \apred \Rightarrow \hrng \Rightarrow \bpred
     }{
     \issubtype{\env,\envBind{x}{\tya}}{\{v:\beta \mid \hrng\}}{\tyb}
     }
}{
  \issubtype{\env}{\hTy}{\typExtF{\tya}{\tyb}}
}[\subh]
$$
\end{adjustbox}

\vspace*{0.5em}

\begin{adjustbox}{max size={\textwidth}{\textheight}}
$$
\inference{
    \inference{
        \apred \Rightarrow \kdom
    }{
    \issubtype{\env}{\tya}{\{v:\alpha \mid \kdom\}}
     } && 
     \inference{
        \apred \Rightarrow \krng \Rightarrow \bpred
     }{
     \issubtype{\env,\envBind{x}{\tya}}{\{v:\beta \mid \krng\}}{\tyb}
     }
}{
  \issubtype{\env}{\kTy}{\typExtF{\tya}{\tyb}}
}[\subk]
$$
\end{adjustbox}

\vspace*{0.5em}

%\begin{adjustbox}{max size={\textwidth}{\textheight}}
$$
\inference{
    \inference{
        \apred \Rightarrow \texttt{true}
    }{
    \issubtype{\env}{\tya}{\alpha}
     } && 
     \inference{
        \apred \Rightarrow p \Rightarrow \bEq{h\ x}{k\ x}
     }{
     \issubtype{\env,\envBind{x}{\tya}}{\propExpr{p}}{\propExpr{\bEq{h\ x}{k\ x}}}
     }
}{
  \issubtype{\env}{\lemmaTy}{\typeExtProp{\tya}{\tyb}{\hName}{\kName}}
}[\sublemma]
$$
%\end{adjustbox}

\vspace*{0.5em}
\noindent \textit{Definitions}\hfill
\vspace*{0.1em}
$$
\begin{array}{rcll}
\typ_g & \doteq & \multicolumn{2}{l}{\typExtG{\tya}{\tyb}}\\
\env & \doteq &  \{ & \envBind{\extName}{\typExt}\\
      &&          , & \envBind{\hName}{\hTy}, \envBind{\kName}{\kTy} \\
      &&          , & \envBind{\lemmaName}{\lemmaTy},  \envBind{\dName}{\dTy} \quad \}\\
\end{array}
$$

\vspace*{0.5em}
\noindent \textit{Derivation Structure}\hfill
\vspace*{0.1em}
\begin{adjustbox}{max size={\textwidth}{\textheight}}
$$
\inference{
    \inference{
        \inference{ 
            {\fbox{\subh}} && \dots 
            }{
        \hastype{\env}{\expr}{\tfuns{\tfun{g}{\typ_g}{(\typeExtProp{\tya}{tyb}{\hName}{g})}}{\propExpr{\fEq{h}{g}}}}
        } && 
        {\fbox{\subk}} && \dots 
        }{
    \hastype{\env}{\expr\ \kName}{(\typeExtProp{\tya}{tyb}{\hName}{\kName}) \rightarrow \propExpr{\fEq{h}{k}}}
    } && 
    {\fbox{\sublemma}} && \dots 
}{
    \hastype{\env}{\underbrace{\extName\ \tyApp{\tya}\ \tyApp{\tyb}\ \dName \ \hName}_{\expr}\ \kName \ \lemmaName}{\propExpr{\fEq{h}{k}}}
}
$$
\end{adjustbox}
\caption{Part of type checking of naive extensionality in \texttt{theoremEq} (see full in Appendix~Fig.~\ref{fig:extensionality-checking-full}).}
\label{fig:extensionality-checking}
\end{figure}


==> proof-current.tex <==
%auto-ignore
\subsection{Type Soundness}\label{sec:proofs-soundness}



We define semantic subtyping as follows: 
\issemsubtype{\env}{\typ}{\typ'} \text{iff} $\forall \model \in \interp{\env}. \interp{\modelapp{\model}{\typ}} \subseteq \interp{\modelapp{\model}{\typ'}}$.
\begin{theorem}[Subtyping semantic soundness]\label{proofs-thm:subsoundness}
  If \issubtype{\env}{\typ}{\typ'} then \issemsubtype{\env}{\typ}{\typ'}.
  %
\begin{proof}
  By induction on the derivation tree: 
  \begin{itemize}
    \item[\subBase]
    Assume \issubtype{\env}{\tref{\rbind}{\tbase}{\refa}}{\tref{\rbind'}{\tbase}{\refa'}}. 
    By inversion 
    $\forall \model\in\interp{\env},~ \interp{\modelapp{\model}{\tref{\rbind}{\tbase}{\refa}}}
      \subseteq \interp{\modelapp{\model}{\tref{\rbind'}{\tbase}{\refa'}}}$, which exactly leads to the required. 
    \item[\subFun]
    Assume \issubtype{\env}{\tfun{x}{\typ_x}{\typ}}{\tfun{x}{\typ'_x}{\typ'}}. 
    By inversion 
    \begin{enumerate}
      \item \issubtype{\env}{\typ'_x}{\typ_x}
      \item \issubtype{\env, \envBind{x}{\typ'_x}}{\typ}{\typ'}
    \end{enumerate}
    By IH 
    \begin{enumerate}
      \setcounter{enumi}{2}
      \item \issemsubtype{\env}{\typ'_x}{\typ_x}
      \item \issemsubtype{\env, \envBind{x}{\typ'_x}}{\typ}{\typ'}
    \end{enumerate}
    We fix $\model\in \env$. 
    We pick $\expr$. We assume $\expr \in \interp{\modelapp{\model}{\tfun{x}{\typ_x}{\typ}}}$ 
    and we will show that $\expr \in \interp{\modelapp{\model}{\tfun{x}{\typ'_x}{\typ'}}}$.
    By assumption $\forall \expr_x \in \interp{\typ_x}\!.\ \expr\ \expr_x \in \interp{\typ\subst{x}{\expr_x}}$. 
    By (3) if $\expr_x \in \interp{\typ_x}$, then $\expr_x \in \interp{\typ'_x}$. 
    By which and (4) $\expr\ \expr_x \in \interp{\typ'\subst{x}{\expr_x}}$. 
    Thus, $\expr \in \interp{\modelapp{\model}{\tfun{x}{\typ'_x}{\typ'}}}$.
    This leads to $\interp{\modelapp{\model}{\tfun{x}{\typ_x}{\typ}}} \subseteq \interp{\modelapp{\model}{\tfun{x}{\typ'_x}{\typ'}}}$, 
    which by definition gives semantic subtyping: 
    \issemsubtype{\env}{\tfun{x}{\typ_x}{\typ}}{\tfun{x}{\typ'_x}{\typ'}}.
    \item[\subEq]  
    Assume \issubtype{\env}{\eqrt{\typ}{\expr_l}{\expr_r}}{\eqrt{\typ'}{\expr_l}{\expr_r}}. 
    By inversion of the rule we have 
    \begin{enumerate}
      \item \issubtype{\env}{\typ}{\typ'} and \issubtype{\env}{\typ'}{\typ}
    \end{enumerate}
    By IH 
    \begin{enumerate}
      \setcounter{enumi}{1}
      \item \issemsubtype{\env}{\typ}{\typ'} and \issemsubtype{\env}{\typ'}{\typ}
    \end{enumerate}
    We fix $\model\in \env$ and we get 
    \begin{enumerate}
      \setcounter{enumi}{2}
      \item \interp{\modelapp{\model}{\typ}} = \interp{\modelapp{\model}{\typ'}}
    \end{enumerate}
    By which and Lemma~\ref{lemma:semantic-sub-eq}
    \begin{enumerate}
      \setcounter{enumi}{3}
      \item \interp{\modelapp{\model}{\eqrt{\typ}{\expr_l}{\expr_r}}} = \interp{\modelapp{\model}{\eqrt{\typ'}{\expr_l}{\expr_r}}}
    \end{enumerate}
    So, trivially, \issemsubtype{\env}{\eqrt{\typ}{\expr_l}{\expr_r}}{\eqrt{\typ'}{\expr_l}{\expr_r}}
  \end{itemize}
\end{proof}
\end{theorem}


\begin{lemma}\label{lemma:semantic-sub-eq}
  If \interp{\typ_i} = \interp{\typ_i'}, then 
  \interp{\eqrt{\typ_i}{\expr_l}{\expr_r}} = \interp{\eqrt{\typ_i'}{\expr_l}{\expr_r}}.
\end{lemma}
\begin{proof}
  We split cases on the structure of $\typ_i$. 
  \begin{itemize}
    \item \textit{If } $\typ_i$ { is a basic type}, then $\typ_i$ is trivially refined to true. 
          Thus, $\typ_i = \typ_i' = \tbase$ and  
          trivially $\interp{\eqrt{\typ_i}{\expr_l}{\expr_r}} = \interp{\eqrt{\typ_i'}{\expr_l}{\expr_r}}$. 
    \item \textit{If } $\typ_i$ { is a function type}, thus 
          \issubtype{\env}{\eqrt{\tfun{x}{\typ_x}{\typ}}{\expr_l}{\expr_r}}{\eqrt{\tfun{x}{\typ'_x}{\typ'}}{\expr_l}{\expr_r}}
  \end{itemize}
  By inversion 
  \begin{enumerate}
    \item \issubtype{\env}{\tfun{x}{\typ_x}{\typ}}{\tfun{x}{\typ'_x}{\typ'}}
    \item \issubtype{\env}{\tfun{x}{\typ'_x}{\typ'}}{\tfun{x}{\typ_x}{\typ}}
  \end{enumerate}
  By inverting the rules again we have 
  \begin{enumerate}
    \setcounter{enumi}{2}
    \item \issubtype{\env}{\typ'_x}{\typ_x}
    \item \issubtype{\env}{\typ_x}{\typ'_x}
    \item \issubtype{\env, \envBind{x}{\typ'_x}}{\typ}{\typ'}
    \item \issubtype{\env, \envBind{x}{\typ_x}}{\typ'}{\typ}
  \end{enumerate}

  We fix $\model\in\interp{\env}$. We need to show that for some $\expr$, 
  if $\expr \in \interp{\modelapp{\model}{\eqrt{\tfun{x}{\typ_x}{\typ}}{\expr_l}{\expr_r}}}$, 
  then $\expr \in \interp{\modelapp{\model}{\eqrt{\tfun{x}{\typ'_x}{\typ'}}{\expr_l}{\expr_r}}}$.
  By assumption we have 
  \begin{enumerate}
    \setcounter{enumi}{6}
    \item  \hasbtype{}{\expr}{\eqt{\unrefine{\tfun{x}{\typ_x}{\typ}}}}
    \item \goesto{\expr}{\exeqName_{\_}\ ({\modelapp{\model}{\expr_l}})\ (\modelapp{\model}{\expr_r})\ {\expr_{pf}}}
    \item ${\modelapp{\model}{\expr_l}}, \modelapp{\model}{\expr_r} \in \interp{\modelapp{\model}{\tfun{x}{\typ_x}{\typ}}}$ 
    \item $\forall \expr_x\in\interp{\modelapp{\model}{\typ_x}}. \expr_{pf}\ \expr_x \in \interp{\eqrt{\typ\subst{x}{\expr_x}}{{\modelapp{\model}{\expr_l}}\ \expr_x}{\modelapp{\model}{\expr_r}\ \expr_x}}$
  \end{enumerate}
  The condition (7) only depend on the structure (and not the refinements) of the types, thus we have. 
  \begin{enumerate}
    \setcounter{enumi}{10}
    \item  \hasbtype{}{\expr}{\eqt{\unrefine{\tfun{x}{\typ'_x}{\typ'}}}}
  \end{enumerate}
  By (9) and IH on (2) we have 
  \begin{enumerate}
    \setcounter{enumi}{11}
    \item ${\modelapp{\model}{\expr_l}}, \modelapp{\model}{\expr_r} \in \interp{\modelapp{\model}{\tfun{x}{\typ'_x}{\typ'}}}$ 
  \end{enumerate}
\end{proof}


==> proofs-contextual.tex <==
%auto-ignore
\subsection{Contextual equivalence}\label{sec:proofs-contextual}

\begin{figure}

\[ \ctx ::= 
  \bullet \mid \ctx\ e \mid e\ \ctx \mid \elam{x}{\typ}{\ctx} \mid 
  \ebeq{\tbase}\ \expr_l\ \expr_r\ \ctx \mid 
  \exeq{x}{\typ_x}{\typ}\ \expr_l\ \expr_r\ \ctx 
\]

\hfill \fbox{\hastype{\env}{\ctx}{\tfun{x}{\typ_x}{\typ}}}

$$
\inference{\iswellformed{\env}{\typ_x}}{
    \hastype{\env}{\bullet}{\tfun{x}{\typ_x}{\typ_x}}
}[\cbullet]
\quad
\inference{
    \hastype{\env, \envBind{y}{\typ_y}}{\ctx}{\tfun{x}{\typ_x}{\typ}} && 
    \iswellformed{\env}{\typ_y}
}{
    \hastype{\env}{\elam{y}{\typ_y}{\ctx}}{\tfun{x}{\typ_x}{\tfun{y}{\typ_y}{\typ}}}
}[\clam]
$$

$$
\inference{    
    \hastype{\env}{\ctx}{\tfun{x}{\typ_x}{\tfun{y}{\typ_y}{\typ}}} && 
    \hastype{\env}{\expr}{\typ}
}{
    \hastype{\env}{\ctx\ \expr}{\tfun{x}{\typ_x}{\typ\subst{y}{\expr}}}
}[\cappl]
\quad
\inference{    
    \hastype{\env}{\expr}{\tfun{y}{\typ_y}{\typ}} && 
    \hastype{\env}{\ctx}{\tfun{x}{\typ_x}{\typ_y}}
}{
    \hastype{\env}{\expr\ \ctx}{\tfun{x}{\typ_x}{\typ\subst{y}{\expr_y}}}
}[\cappr]
$$


$$
\eqcolor{
\inference{
 \hastype{\env}{\expr_l}{\typ_l} && 
 \hastype{\env}{\expr_r}{\typ_r} &&
 \issubtype{\env}{\typ_r}{\tref{y}{\tbase}{\etrue}} && 
 \issubtype{\env}{\typ_l}{\tref{y}{\tbase}{\etrue}} \\  
 \hastype{\env, \envBind{r}{\typ_r}, \envBind{l}{\typ_l}}{\ctx}{\tfun{x}{\typ_x}{\tref{\rbind}{\tunit}{\bbbeq{l}{r}{\tbase}}}}
}{
  \hastype{\env}{\ebeq{\tbase}\ \expr_l\ \expr_r\ \ctx}{\tfun{x}{\typ_x}{\eqrt{\tbase}{\expr_l}{\expr_r}}}
}[\ceqbase]
}
$$

$$
\eqcolor{
\inference{
 \hastype{\env}{\expr_l}{\typ_l} && 
 \hastype{\env}{\expr_r}{\typ_r} &&
 \issubtype{\env}{\typ_l}{\tfun{y}{\typ_y}{\typ}} && 
 \issubtype{\env}{\typ_r}{\tfun{y}{\typ_y}{\typ}} \\  
 \hastype{\env, \envBind{r}{\typ_r}, \envBind{l}{\typ_l}}{\ctx}{(\tfun{x}{\typ_x}{\tfun{y}{\typ_y}{\eqrt{\typ}{l\ x}{r\ x}}})} && 
 \iswellformed{\env}{\tfun{y}{\typ_y}{\typ}}
}{
  \hastype{\env}{\exeq{y}{\typ_y}{\typ}\ \expr_l\ \expr_r\ \ctx}{\tfun{x}{\typ_x}{\eqrt{\tfun{y}{\typ_y}{\typ}}{\expr_l}{\expr_r}}}
}[\ceqfun]
}
$$

\caption{Contexts and their typing.}
\label{fig:contexts}
\end{figure}

\begin{lemma}[Context application is well typed]\label{lem:ctx-app}
  If \hastype{\env}{\ctx}{\tfun{x}{\typ_x}{\typ}} and
  \hastype{\env}{\expr}{\typ_x} then
  \hastype{\env}{\ctxapp{\ctx}{\expr}}{\typ\subst{x}{\expr}}.
%
\begin{proof}
  By induction on \ctx's typing derivation. \todo{...}
\end{proof}  
\end{lemma}

\begin{theorem}[LR is congruence closed]\label{thm:lr-contextual}
   If \hastype{\env}{\ctx}{\tfun{x}{\typ_x}{\typ}} and
   \relatesEnv{\env}{\expr_l}{\expr_r}{\typ_x}, then
   \relatesEnv{\env}{\ctxapp{\ctx}{\expr_l}}{\ctxapp{\ctx}{\expr_r}}{\typ\subst{x}{\expr_l}}.
%
\begin{proof}
  By induction on \ctx's typing derivation.
  \todo{... should look like the fundamental theorem}
\end{proof}
\end{theorem}

\begin{theorem}[PEq is congruence closed]\label{thm:peq-contextual}
   If \hastype{\env}{\ctx}{\tfun{x}{\typ_x}{\typ}} and
   \hastype{\env}{\expr}{\eqrt{\typ_x}{\expr_l}{\expr_r}} then
   there exists $\expr'$ such that
   \hastype{\env}{\expr'}{\eqrt{\typ\subst{x}{\expr_l}}{\ctxapp{\ctx}{\expr_l}}{\ctxapp{\ctx}{\expr_r}}}.
%
\begin{proof}
  By induction on \typ.
%
\begin{itemize}
\item $\typ \doteq \tref{y}{\tbase}{\refa}$.
%
\begin{enumerate}
\item Let $\expr' = \ebeq{\tbase}\ \ctxapp{\ctx}{\expr_l}\ \ctxapp{\ctx}{\expr_r}\ \eunit$. 
\item By \teqbase, with $\typ_l =
  \tref{x}{\tbase}{\bbbeq{x}{\ctxapp{\ctx}{\expr_l}}{\tbase}}$ and similarly
    for $\typ_r$. We must show:
%
  \subitem \hastype{\env}{\ctxapp{\ctx}{\expr_l}}{\tref{x}{\tbase}{\bbbeq{x}{\ctxapp{\ctx}{\expr_l}}{\tbase}}}
  \subitem \hastype{\env}{\ctxapp{\ctx}{\expr_r}}{\tref{x}{\tbase}{\bbbeq{x}{\ctxapp{\ctx}{\expr_r}}{\tbase}}}
  \subitem \issubtype{\env}{\typ_r}{\tref{x}{\tbase}{\etrue}}
  \subitem \issubtype{\env}{\typ_l}{\tref{x}{\tbase}{\etrue}}
  \subitem \hastype{\env, \envBind{r}{\typ_r}, \envBind{l}{\typ_l}}{\expr}{\tref{\rbind}{\tunit}{\bbbeq{l}{r}{\tbase}}}
\item We find the first two by \tself.
\item We find the next two by \subBase.
\item \todo{hmm... not quite. we need this to look like reflexivity, using \pfty}
\end{enumerate}
  
\item $\typ \doteq \tfun{y}{\typ_y}{\typ'}$.
%
\qedhere
\end{itemize}
\end{proof}
\end{theorem}

